A Survey of Generative Categories and Techniques in Multimodal Generative Models

Multimodal generative models (MGMs) have rapidly expanded beyond text generation to encompass images, music, video, human motion, and 3D objects. This survey categorises six primary text-conditioned generative modalities and examines how four techniques, namely self-supervised learning, mixture of experts, reinforcement learning from human feedback, and chain-of-thought prompting, are adapted across them, distinguishing shared mechanisms from experimentally supported benefits. We organise evaluation around faithfulness, compositionality, and robustness, and interpret evidence within each study's protocol. Selected within-study comparisons reported in the reviewed literature support four findings: preference gains need not improve text relevance, and reward optimisation can reduce within-prompt diversity; intermediate plans require tests of their realisation in final outputs; expert granularity changes the mechanism and its storage, computation, and runtime costs; and gains against an optimisation score need confirmation outside that scoring path. We further analyse trustworthiness risks, including bias, privacy leakage, and misuse of generated media, and examine the evidence for mitigation strategies.

==> Definitions/journalnames.tex <==
% Updated 05 January 2026 used for Y2026
%% --------------------------------------------------------------------
%\DeclareOption{}{%%
%		\gdef\@journal{}
%		\gdef\@journalfull{}
%		\gdef\@journalshort{}
%		\gdef\@doiabbr{}
%		\gdef\@ISSN{}
%		\gdef\@societyowner{}
%}
%% --------------------------------------------------------------------
%% Fields meanings:
%% - Option name: Journal website name (used in URL)
%% - @journal: Journal website name (used in URL)
%% - @journalshort: Short Name (ISO4)
%% - @journalfull: Journal full name
%% - @doiabbr: DOI abbreviation of the journal used in DOI numbers 10.32604/journalnameXXXX
%% - @ISSN: Journal E-ISSN number
%% - @continuouspages: use  for journals that use pagination
%% - @societyowner: Name of society owning the journal (for society journals)
%% --------------------------------------------------------------------
\DeclareOption{biocell}{%
	\gdef\@journal{biocell}
	\gdef\@journalshort{Biocell}
	\gdef\@journalfull{Biocell}
	\gdef\@doiabbr{biocell}
	\gdef\@ISSN{1667-5746}
	\gdef\@societyowner{}
}
\DeclareOption{chd}{%
	\gdef\@journal{chd}
	\gdef\@journalshort{Congenit Heart Dis}
	\gdef\@journalfull{Congenital Heart Disease}
	\gdef\@doiabbr{chd}
	\gdef\@ISSN{1747-0803}
	\gdef\@societyowner{}
}
\DeclareOption{cju}{%
	\gdef\@journal{cju}
	\gdef\@journalshort{Can J Urol}
	\gdef\@journalfull{Canadian Journal of Urology}
	\gdef\@doiabbr{cju}
	\gdef\@ISSN{1488-5581}
	\gdef\@societyowner{}
}
\DeclareOption{cl}{%
	\gdef\@journal{cl}
	\gdef\@journalshort{Chalcogenide Lett}
	\gdef\@journalfull{Chalcogenide Letters}
	\gdef\@doiabbr{cl}
	\gdef\@ISSN{1584-8663}
	\gdef\@societyowner{}
}
\DeclareOption{cmc}{%
 	\gdef\@journal{cmc}
	\gdef\@journalshort{Comput Mater Contin}
	\gdef\@journalfull{Computers, Materials \& Continua}
	\gdef\@doiabbr{cmc}
	\gdef\@ISSN{1546-2226}
	\gdef\@societyowner{}
}
\DeclareOption{cmes}{%
 	\gdef\@journal{cmes}
	\gdef\@journalshort{Comput Model Eng Sci}
	\gdef\@journalfull{Computer Modeling in Engineering \& Sciences}
	\gdef\@doiabbr{cmes}
	\gdef\@ISSN{1526-1506}
	\gdef\@societyowner{}
}
\DeclareOption{csse}{%
 	\gdef\@journal{csse}
	\gdef\@journalshort{Comput Syst Sci Eng}
	\gdef\@journalfull{Computer Systems Science and Engineering}
	\gdef\@doiabbr{csse}
	\gdef\@ISSN{0267-6192}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{dedt}{%
 	\gdef\@journal{dedt}
	\gdef\@journalshort{Digit Eng Digit Twin}
	\gdef\@journalfull{Digital Engineering and Digital Twin}
	\gdef\@doiabbr{dedt}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{ecn}{%
 	\gdef\@journal{ecn}
	\gdef\@journalshort{Eur Cytokine Netw}
	\gdef\@journalfull{European Cytokine Network}
	\gdef\@doiabbr{ecn}
	\gdef\@ISSN{1952-4005}
	\gdef\@societyowner{}
}
\DeclareOption{ee}{%
 	\gdef\@journal{ee}
	\gdef\@journalshort{Energy Eng}
	\gdef\@journalfull{Energy Engineering}
	\gdef\@doiabbr{ee}
	\gdef\@ISSN{1546-0118}
	\gdef\@societyowner{}
}
\DeclareOption{fdmp}{%
 	\gdef\@journal{fdmp}
	\gdef\@journalshort{Fluid Dyn Mater Process}
	\gdef\@journalfull{Fluid Dynamics \& Materials Processing}
	\gdef\@doiabbr{fdmp}
	\gdef\@ISSN{1555-2578}
	\gdef\@societyowner{}
}
\DeclareOption{fhmt}{%
 	\gdef\@journal{fhmt}
	\gdef\@journalshort{Front Heat Mass Transf}
	\gdef\@journalfull{Frontiers in Heat and Mass Transfer}
	\gdef\@doiabbr{fhmt}
	\gdef\@ISSN{2125-8629}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{iasc}{%
 	\gdef\@journal{iasc}
	\gdef\@journalshort{Intell Autom Soft Comput}
	\gdef\@journalfull{Intelligent Automation \& Soft Computing}
	\gdef\@doiabbr{iasc}
	\gdef\@ISSN{2326-005X}
	\gdef\@societyowner{}
}
\DeclareOption{icces}{%
 	\gdef\@journal{icces}
	\gdef\@journalshort{Int Conf Comput Exp Eng Sci}
	\gdef\@journalfull{The International Conference on Computational \& Experimental Engineering and Sciences}
	\gdef\@doiabbr{icces}
	\gdef\@ISSN{1993-2815}
	\gdef\@societyowner{}
}
\DeclareOption{ijmhp}{%
 	\gdef\@journal{ijmhp}
	\gdef\@journalshort{Int J Ment Health Promot}
	\gdef\@journalfull{International Journal of Mental Health Promotion}
	\gdef\@doiabbr{ijmhp}
	\gdef\@ISSN{2049-8543}
	\gdef\@societyowner{}
}
\DeclareOption{jai}{%
 	\gdef\@journal{jai}
	\gdef\@journalshort{J Artif Intell}
	\gdef\@journalfull{Journal on Artificial Intelligence}
	\gdef\@doiabbr{jai}
	\gdef\@ISSN{2579-003X}
	\gdef\@societyowner{}
}
\DeclareOption{jbd}{%
 	\gdef\@journal{jbd}
	\gdef\@journalshort{J Big Data}
	\gdef\@journalfull{Journal on Big Data}
	\gdef\@doiabbr{jbd}
	\gdef\@ISSN{2579-0056}
	\gdef\@societyowner{}
}
\DeclareOption{jbic}{%
 	\gdef\@journal{jbic}
	\gdef\@journalshort{J Blockchain Intell Comput}
	\gdef\@journalfull{Journal of Blockchain and Intelligent Computing}
	\gdef\@doiabbr{jbic}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{jcs}{%
 	\gdef\@journal{jcs}
	\gdef\@journalshort{J Cyber Secur}
	\gdef\@journalfull{Journal of Cyber Security}
	\gdef\@doiabbr{jcs}
	\gdef\@ISSN{2579-0064}
	\gdef\@societyowner{}
}
\DeclareOption{jihpp}{%
 	\gdef\@journal{jihpp}
	\gdef\@journalshort{J Inf Hiding Priv Prot}
	\gdef\@journalfull{Journal of Information Hiding and Privacy Protection}
	\gdef\@doiabbr{jihpp}
	\gdef\@ISSN{2637-4226}
	\gdef\@societyowner{}
}
\DeclareOption{jimh}{%
 	\gdef\@journal{jimh}
	\gdef\@journalshort{JIMH}
	\gdef\@journalfull{Journal of Intelligent Medicine and Healthcare}
	\gdef\@doiabbr{jimh}
	\gdef\@ISSN{2837-634X}
	\gdef\@societyowner{}
}
\DeclareOption{jiot}{%
 	\gdef\@journal{jiot}
	\gdef\@journalshort{J Internet Things}
	\gdef\@journalfull{Journal on Internet of Things}
	\gdef\@doiabbr{jiot}
	\gdef\@ISSN{2579-0080}
	\gdef\@societyowner{}
}
\DeclareOption{jnm}{%
 	\gdef\@journal{jnm}
	\gdef\@journalshort{J New Media}
	\gdef\@journalfull{Journal of New Media}
	\gdef\@doiabbr{jnm}
	\gdef\@ISSN{2579-0129}
	\gdef\@societyowner{}
}
\DeclareOption{jpa}{%
 	\gdef\@journal{jpa}
	\gdef\@journalshort{J Psychol Afr}
	\gdef\@journalfull{Journal of Psychology in Africa}
	\gdef\@doiabbr{jpa}
	\gdef\@ISSN{1815-5626}
	\gdef\@societyowner{}
}
\DeclareOption{jpm}{%
 	\gdef\@journal{jpm}
	\gdef\@journalshort{J Polym Mater}
	\gdef\@journalfull{Journal of Polymer Materials}
	\gdef\@doiabbr{jpm}
	\gdef\@ISSN{0976-3449}
	\gdef\@societyowner{}
}
\DeclareOption{jqc}{%
 	\gdef\@journal{jqc}
	\gdef\@journalshort{J Quantum Comput}
	\gdef\@journalfull{Journal of Quantum Computing}
	\gdef\@doiabbr{jqc}
	\gdef\@ISSN{2579-0145}
	\gdef\@societyowner{}
}
\DeclareOption{jrm}{%
 	\gdef\@journal{jrm}
	\gdef\@journalshort{J Renew Mater}
	\gdef\@journalfull{Journal of Renewable Materials}
	\gdef\@doiabbr{jrm}
	\gdef\@ISSN{2164-6341}
	\gdef\@societyowner{}
}
\DeclareOption{oncologie}{%
 	\gdef\@journal{oncologie}
	\gdef\@journalshort{Oncologie}
	\gdef\@journalfull{Oncologie}
	\gdef\@doiabbr{oncologie}
	\gdef\@ISSN{1765-2839}
	\gdef\@societyowner{}
}
\DeclareOption{or}{%
 	\gdef\@journal{or}
	\gdef\@journalshort{Oncol Res}
	\gdef\@journalfull{Oncology Research}
	\gdef\@doiabbr{or}
	\gdef\@ISSN{1555-3906}
	\gdef\@societyowner{}
}
\DeclareOption{phyton}{%
 	\gdef\@journal{phyton}
	\gdef\@journalshort{Phyton-Int J Exp Bot}
	\gdef\@journalfull{Phyton-International Journal of Experimental Botany}
	\gdef\@doiabbr{phyton}
	\gdef\@ISSN{1851-5657}
	\gdef\@societyowner{}
}
\DeclareOption{rig}{%
 	\gdef\@journal{rig}
	\gdef\@journalshort{Rev Int Géomatique}
	\gdef\@journalfull{Revue Internationale de Géomatique}
	\gdef\@doiabbr{rig}
	\gdef\@ISSN{2116-7060}
	\gdef\@societyowner{}
}
\DeclareOption{rimni}{%
 	\gdef\@journal{rimni}
	\gdef\@journalshort{Revista Internacional de Métodos Numéricos para Cálculo y Diseño en Ingeniería}
	\gdef\@journalfull{Rev Int méTodos Numér Cálc Diseño Ing}
	\gdef\@doiabbr{rimni}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{sdhm}{%
 	\gdef\@journal{sdhm}
	\gdef\@journalshort{Struct Durab Health Monit}
	\gdef\@journalfull{Structural Durability \& Health Monitoring}
	\gdef\@doiabbr{sdhm}
	\gdef\@ISSN{1930-2991}
	\gdef\@societyowner{}
}
\DeclareOption{zkg}{%
 	\gdef\@journal{zkg}
	\gdef\@journalshort{ZKG Int}
	\gdef\@journalfull{ZKG International}
	\gdef\@doiabbr{zkg}
	\gdef\@ISSN{2366-1313}
	\gdef\@societyowner{}
}
\DeclareOption{notspecified}{%
	\gdef\@journal{notspecified}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{journal}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{test}{%
	\gdef\@journal{test}
	\gdef\@journalfull{TEST}
	\gdef\@journalshort{TEST}
	\gdef\@doiabbr{test}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
